La conjecture de Mordell: origines, approches, g\'en\'eralisations

The Mordell conjecture: origins, approaches, generalizations -- The Mordell conjecture predicts that a diophantine equation defining a smooth projective curve of genus at least two has only finity many solutions in a given number field. The century that ran since its statement, in 1922, gave rise to several approaches, several proofs, and vast extensions most of which are still conjectural. This text is based on the oral presentation and aims at recalling this story. La conjecture de Mordell pr\'edit qu'une \'equation diophantienne d\'efinissant une courbe projective lisse de genre au moins deux n'a qu'un nombre fini de solutions dans un corps de nombres donn\'e. Le si\`ecle qui s'est \'ecoul\'e depuis son \'enonc\'e, en 1922, a vu plusieurs approches, plusieurs d\'emonstrations, ainsi que de vastes extensions dont la plupart sont encore conjecturales. Ce texte, qui reprend l'expos\'e oral, s'efforce de retracer cette histoire.

==> frenchbst.tex <==
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{\'editeurs}        \def\bbleds{\'eds.}
\def\bbleditor{\'editeur}          \def\bbled{\'ed.}
\def\bbledby{\'edit\'e by}
\def\bbledition{\'edition}        \def\bbledn{\'ed.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n\textsuperscript o}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{p.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Pr\'epublication}
\def\bbltechrep{Pr\'ep.}
\def\bblmthesis{M\'emoire de DEA}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1\textsuperscript{re}}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\textsuperscript{e}}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\textsuperscript{e}}
\def\bblfourth{Fourth}          \def\bblfourtho{4\textsuperscript{e}}
\def\bblfifth{Fifth}            \def\bblfiftho{5\textsuperscript{e}}
\def\bblst{\textsuperscript{re}}
  \def\bblnd{\textsuperscript{e}}  \def\bblrd{\textsuperscript{e}}
\def\bblth{\textsperscript{e}}
\def\bbljan{Janvier}  \def\bblfeb{F\'evrier}  \def\bblmar{Mars}
\def\bblapr{Avril}    \def\bblmay{Mai}       \def\bbljun{Juin}
\def\bbljul{Juillet}     \def\bblaug{Ao\^ut}    \def\bblsep{Septembre}
\def\bbloct{Octobre}  \def\bblnov{Novembre}  \def\bbldec{Decembre}


